Semi-Explicit Solution of Some Discrete-Time Mean-Field-Type Games with Higher-Order Costs

Traditional solvable game theory and mean-field-type game theory (risk-aware games) predominantly focus on quadratic costs due to their analytical tractability. Nevertheless, they often fail to capture critical non-linearities inherent in real-world systems. In this work, we present a unified framework for solving discrete-time game problems with higher-order state and strategy costs involving power-law terms. We derive semi-explicit expressions for equilibrium strategies, cost-to-go functions, and recursive coefficient dynamics across deterministic, stochastic, and multi-agent system settings by convex-completion techniques. The contributions include variance-aware solutions under additive and multiplicative noise, extensions to mean-field-type-dependent dynamics, and conditions that ensure the positivity of recursive coefficients. Our results provide a foundational methodology for analyzing non linear multi-agent systems under higher-order penalization, bridging classical game theory and mean-field-type game theory with modern computational tools for engineering applications.

==> MacrosMatematicas.tex <==
\makeatletter
\iflibroproyecto
%-------------------------Los elementos a,b,c,d---------------------------------------
\glossary(Elementos){$a$, $b$, $c$, $d$}{Elementos}%
%-------------------------Las variables w,x,y,z---------------------------------------
\glossary(Variables){$t$, $w$, $x$, $y$, $z$}{Variables}%
%-------------------------Los parámetros p,q,r,s--------------------------------------
\glossary(Parametros){$\alpha,\beta,\chi,\ldots$}{Parámetros}%
%-------------------------Variables índice y enteras--------------------------------------
\glossary(VariablesIndiceYEnteras){$i$, $j$, $k$, $l$, $m$, $n$}{Variables índice y enteras}%
\fi
%-------------------------El conjunto {a,b,c,d,...} de elementos a,b,c,d...-----------
\newcommand{\CtoEtos}[1]{\left\{\kern0.5pt #1\kern0.5pt\right\}}%
\iflibroproyecto
\glossary(ConjuntoElementos)%
{$\CtoEtos{a,b,c,\ldots}$}%
{Conjunto de los elementos $a$, $b$, $c$, $\ldots$}%
\fi
%-------------------------Conjunto de los a tales que P(a) {a|P}----------------------
\newcommand{\CtoPdadP}[2]{\CtoEtos{#1\mid #2}}%
\iflibroproyecto
\glossary(ConjuntoPropiedadP)%
{$\CtoPdadP{a}{P(a)}$}%
{Conjunto de los elementos $a$ con la propiedad $P(a)$}%
\fi
%-------------------------Conjuntos---------------------------------------------------
\newcommand{\Cto}[1]{\MakeUppercase{#1}}%
\iflibroproyecto
\glossary(Conjuntos){$\Cto{A}$, $\Cto{B}$, $\Cto{C}$, $\ldots$}{Conjuntos}%
\fi
%-------------------------Conjunto potencia-------------------------------------------
\newcommand{\CtoP}[1]{\mathcal{P}\left(\Cto{#1}\right)}%
\iflibroproyecto
\glossary(ConjuntoPotencia){$\CtoP{A}$}{Conjunto potencia de $\Cto{A}$}%
\fi
% ---------------------------Clase de Conjuntos (conjunto de conjuntos) ---------------------------
\newcommand{\ClsCto}[2]{\mathcal{#1}\left(\Cto{#2}\right)}%
\newcommand{\ClaseCto}[1]{\mathcal{#1}}%
\iflibroproyecto
\glossary(ClaseDeConjuntos)
{$\ClsCto{A}{B}$, $\ClaseCto{A}$}
{Clases de conjuntos (conjuntos de conjuntos)}%
\fi
%%\newcommand{\CtoPX}{\CtoP{\CtoX}}%
%  Conjunto potencia borroso
%%\newcommand{\CtoF}{\mathcal{F}\left(\CtoX\right)}%
% ---------------------------Complemento de un conjunto ---------------------------
\newcommand{\CCto}[1]{\overline{#1}}%
\iflibroproyecto
\glossary(ConjuntoComplemento){$\CCto{\Cto{A}}$}{Complemento del conjunto $\Cto{A}$}%
\fi
% ------------------Unión e intersección de conjuntos----------------------------------------------
\DeclareRobustCommand{\ICto}{\@ifstar{\bigcap}{\cap}}%
\DeclareRobustCommand{\UCto}{\@ifstar{\bigcup}{\cup}}%
\iflibroproyecto
\glossary(ConjuntosUnion)%
{$\UCto*\Cto{A}_i$, $\Cto{A}\UCto\Cto{B}$}%
{Unión de conjuntos}%
\glossary(ConjuntosInterseccion)%
{$\ICto*\Cto{A}_i$, $\Cto{A}\ICto\Cto{B}$}%
{Intersección de conjuntos}%
\fi
% ------------------Diferencia de conjuntos----------------------------------------------
\iflibroproyecto
\glossary(ConjuntoDiferencia)%
{$\Cto{A}-\Cto{B}$}%
{Conjunto diferencia formado por elementos que están en $\Cto{A}$ y no en $\Cto{B}$}%
\fi
%----------------------------Producto cartesiano de conjuntos--------------------------------------
\newcommand{\PCCto}{\times}%
\iflibroproyecto
\glossary(ProductoCartesiano)
{$\Cto{A}\PCCto\Cto{B}$}
{Producto cartesiano de los conjuntos $\Cto{A}$ y $\Cto{B}$}%
\glossary(ProductoCartesianoNVeces)
{$\Cto{A}^n$}
{Producto cartesiano $\Cto{A}\PCCto\Cto{A}\PCCto\cdots\PCCto\Cto{A}$ $n$ veces}%
\fi
%-----------------Conjunto de los números naturales, enteros y reales----------------------------
\newcommand{\CtoN}{\mathbb{N}}%
\newcommand{\CtoR}{\mathbb{R}}%
\newcommand{\CtoZ}{\mathbb{Z}}%
%\newcommand{\CtoQ}{\mathbb{Q}}%
\iflibroproyecto
\glossary(ConjuntoNaturalesEnterosReales)%
{$\CtoN$, $\CtoZ$, $\CtoR$}%
{Conjunto de naturales $\CtoEtos{1,2,\ldots}$,
enteros $\CtoEtos{\ldots,-1,0,1,\ldots}$ y reales}%
\fi
%------------------------------Conjunto Universal y vacío------------------------------------------
\newcommand{\CtoX}{\Cto{X}}%
\newcommand{\CtoV}{\emptyset}%
\iflibroproyecto
\glossary(ConjuntoUniversalVacio){$\CtoX$, $\CtoV$}{Conjunto universal y vacío}%
\fi
%---------------------------Pertenencia y no pertenencia al conjunto-------------------------------
%\in, \notin
\iflibroproyecto
\glossary(PertenenciaYNoPertenencia){$\in$, $\notin$}{Pertenencia y no pertenencia a un conjunto}%
\fi
%--------------------------Subconjunto y superconjunto---------------------------------------------
%\subseteq, \supseteq, \subset o \supset
\iflibroproyecto
\glossary(SubconjuntoYSuperconjunto)
{$\subseteq$, $\subset$,  $\supseteq$, $\supset$}
{Subconjunto, subconjunto propio, superconjunto, superconjunto propio}%
\fi
% Cardinalidad de un conjunto
%%\newcommand{\Card}[1]{\left|#1\right|}%
%------------------Relación binaria genérica. Subconjunto de AxB.-----------------------------------
\newcommand{\RBin}{R}%
\iflibroproyecto
\glossary(RelacionBinaria){$a\RBin b$}{Elemento $a$ relacionado con $b$ por medio de la relación binaria $\RBin$}%
\fi
%------------------Igualdad y no igualdad-----------------------------------------------------------
% =, \neq 
\iflibroproyecto
\glossary(IgualdadYNoIgualdad){$=$, $\neq$}{Igualdad y no igualdad}%
\fi
%---- Conectores lógicos ``y'', ``o'', ``no'', ``si entonces'', ``si y sólo si''.--------------------
\newcommand{\Cjc}{\text{y}}%
\newcommand{\Dyc}{\text{o}}%
\newcommand{\Neg}{\neg}%
\newcommand{\Imp}{\Rightarrow}%
\newcommand{\Coimp}{\Leftrightarrow}%
\iflibroproyecto
\glossary(ConectoresLogicos){$\Cjc$, $\Dyc$, $\Neg$, $\Imp$, $\Coimp$}
                            {Conectores lógicos ``y'', ``o'', ``no'', ``si entonces'', ``si y sólo si''}%
\fi
%  Cuantificador existencial
%\exists
%  Cuantificador universal
%\forall
%  Descriptor |
% |
% Equivalencia 
%\equiv--G
%------------------------------Relación de orden o desigualdades--------------------------------
% \leq, <, \geq ó >
\iflibroproyecto
\glossary(RelacionesDeOrdenMenorMayor)
{$\leq$, $<$, $\geq$, $>$}
{Relación de orden menor o igual, menor, mayor o igual, mayor}%
\fi
%------------------------------Símbolo de elementos 'incomparables'--------------------------------
\newcommand{\Incomp}{\mid\mid}%
\iflibroproyecto
\glossary(Incomparables){$a\Incomp b$}{Elementos $a$ y $b$ incomparables}%
\fi
% -----------------------------Supremo, ínfimo, máximo y mínimo--------------------------------------
% \max, \min \sup, \inf
\iflibroproyecto
\glossary(MaximoMinimoSupremoInfimo){$\max$, $\min$, $\sup$, $\inf$}{Máximo, mínimo, supremo e ínfimo}%
\fi
%----------------------------Operaciones conjunción y disyunción.-----------------------------
\DeclareRobustCommand{\OpCjc}{\@ifstar{\bigwedge}{\hspace{-0.5pt}\wedge\hspace{-0.5pt}}}%
\DeclareRobustCommand{\OpDyc}{\@ifstar{\bigvee}{\hspace{-0.5pt}\vee\hspace{-0.5pt}}}%
\iflibroproyecto
\glossary(OperacionConjuncionyDisyuncion)%
{$\OpDyc* a_i$, $\OpCjc* a_i$, $a\OpDyc b$, $a\OpCjc b$}{Disyunción y conjunción de elementos}%
\fi
%-------------------------------------Operación complemento------------------------------------------
\DeclareRobustCommand{\OpComp}[1]{#1^\prime}%
\DeclareRobustCommand{\OpCompinf}[1]{\OpComp{\underline{#1}}}%
\DeclareRobustCommand{\OpCompsup}[1]{\OpComp{\overline{#1}}}%
\iflibroproyecto
\glossary(OperacionComplemento){$\OpComp{a}$}{Complemento del elemento $a$}%
\fi
%-------------- El cero y la unidad de un conjunto --------------------------------------------------
\newcommand{\ElCero}{0}%
\newcommand{\LaUnidad}{1}%
\iflibroproyecto
\glossary(CeroYUnidad){$\ElCero$, $\LaUnidad$}{El cero y la unidad}%
\fi
%  Una manera de escribir retículo
%\newcommand{\Reticulo}[1]{\mathfrak{#1}}%--G
%-----Intervalos cerrado-cerrado, cerrado-abierto, abierto-cerrado, abierto-abierto ---------------
\newcommand{\IntCC}[1]{\left[#1\right]}%
\newcommand{\IntCA}[1]{\left[#1\right)}%
\newcommand{\IntAC}[1]{\left(#1\right]}%
\newcommand{\IntAA}[1]{\left(#1\right)}%
\iflibroproyecto
\glossary(Intervalos){$\IntCC{a,b}$, $\IntCA{a,b}$, $\IntAC{a,b}$, $\IntAA{a,b}$}{Intervalos}%
\fi
%-------------------------El Punto fijo del complemento--------------------------------------------
\newcommand{\ElPFC}{e_{c}}%
\iflibroproyecto
\glossary(PuntoFijo){$\ElPFC$}{Punto fijo del complemento}%
\fi
%  Isomorfismo
%%\newcommand{\Isomorfo}{\cong}%
%---------------------------Álgebras en notación A (versión *) ó (A,v,n,',0,1)--------------------
\DeclareRobustCommand{\Alg}{\@ifstar\Alg@i\Alg@ii}%
\DeclareRobustCommand{\Alg@i}[1]{\mathscr{\MakeUppercase{#1}}}%
\DeclareRobustCommand{\Alg@ii}[1]{\nTupla{#1;\OpDyc,\OpCjc,\OpComp{},\ElCero,\LaUnidad}}%
%\DeclareRobustCommand{\Alg@ii}[2][\ElCero,\LaUnidad]{\nTupla{#2\thinspace;\OpDyc,\OpCjc,\OpComp{},#1}}%
\DeclareRobustCommand{\AlgMorgan}[1][]{\Alg*{M}_{#1}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgKleene}[1][]{\Alg*{K}_{#1}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgBoole}[1][]{\Alg*{B}_{#1}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgFormulas}{\Alg*{F}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgTskLdbm}[1][]{\Alg*{T}_{#1}}%--No está en glosario porque ya está \Alg.
\iflibroproyecto
\glossary(Algebras){$\Alg*{A}$, $\Alg*{B}$, $\Alg*{C}$, $\ldots$}{Álgebras}%
\fi
%----------------------------Cociente--------------------------------------------------------------
\newcommand{\Coc}[2]{#1/#2}%
\iflibroproyecto
\glossary(Cociente){$\Coc{}{}$}{Cociente}%
\fi
%----------------------Una manera de escribir fórmula. f,h,g.-------------------------------------
\newcommand{\Frml}[1]{\MakeLowercase{#1}}%
\iflibroproyecto
\glossary(Formulas)%
{$\Frml{f}$, $\Frml{g}$, $\Frml{h}$, $\Frml{p}$, $\Frml{q}$, $\Frml{r}$, $\Frml{s}$}%
{Fórmulas o funciones definidas por fórmulas}%
\fi
%---------------------------Clase de equivalencia--------------------------------------------------
\newcommand{\ClsEquiv}[1]{\left[#1\right]}%
\iflibroproyecto
\glossary(ClaseEquivalencia){$\ClsEquiv{a}$}{Clase de equivalencia que contiene al elemento $a$}%
\fi
%---------------------------Fórmula f equivalente a g en el álgebra -------------------------------
\newcommand{\Fequiv}[1]{\equiv_{_{#1}}\hspace{-1.5pt}}%
\iflibroproyecto
\glossary(EquivalenciaFormula){$\Frml{f}\Fequiv{\Alg*{A}}\Frml{g}$}%
{Fórmulas $\Frml{f}$ y $\Frml{g}$ equivalentes sobre el álgebra $\Alg*{A}$}%
\fi
%  Operador de t-norma
%%\newcommand{\OpTnrm}{\@ifstar{\bigotimes}{\otimes}}%--G
%  Operador de T-conorma
%%\newcommand{\OpTcnrm}{\@ifstar{\bigoplus}{\oplus}}%--G
%  Operador complemento borroso
%%\newcommand{\OpCtoTTc}[1]{#1'}%
%---------------------------Operador de T-norma y T-conorma -------------------------------
\newcommand{\OpTn}{\bigtriangleup}%
\newcommand{\OpTc}{\bigtriangledown}%
\iflibroproyecto
\glossary(TnormaTconorma){$a\OpTc b$, $a\OpTn b$}%
{T-conorma y t-norma de los elementos $a$ y $b$}%
\fi
%---------------------------Operador de complemento difuso -------------------------------
\newcommand{\CompDif}{\@ifstar{\@SCompDif}{\@NSCompDif}}%
\newcommand{\@NSCompDif}[1]{\Lambda\left(#1\right)}%
\newcommand{\@SCompDif}{\Lambda}%
%--------------------- n-Tupla de elementos <x1,x2,...,xn>----------------------------------------
\DeclareRobustCommand{\nTupla}[1]{\left\langle #1\right\rangle}%
\iflibroproyecto
\glossary(Ntupla){$\nTupla{a_1,a_2,\ldots,a_n}$}{$n$-tupla de elementos}%
\fi
%  Vector de elementos [x1,x2,...,xn]
%%\newcommand{\VectorEtos}[1]{\left[#1\right]}%
%--------------------- Forma normal disyuntiva y conjuntiva -------------------------------------
\newcommand{\FND}[2]{\text{\normalfont D}_{_{#2}}(\Frml{#1})}%
\newcommand{\FNC}[2]{\text{\normalfont C}_{_{#2}}(\Frml{#1})}%
\iflibroproyecto
\glossary(FormasNormales)%
{$\FND{f}{\Alg*{A}}$, $\FNC{f}{\Alg*{A}}$}%
{Forma normal disyuntiva y conjuntiva de $\Frml{f}$ en el álgebra $\Alg*{A}$}%
\fi
%--------------------- Expansiones disyuntiva y conjuntiva -------------------------------------
\newcommand{\ED}[3][]{\text{\normalfont ED}_{_{#1}}^{#3}(\Frml{#2})}%
\newcommand{\EC}[3][]{\text{\normalfont EC}_{_{#1}}^{#3}(\Frml{#2})}%
\iflibroproyecto
\glossary(Expansiones)%
{$\ED[{\Alg*{A}}]{f}{x}$, $\EC[{\Alg*{A}}]{f}{x}$}%
{Expansión disyuntiva y conjuntiva de $\Frml{f}$ en $\Alg*{A}$ respecto a $x$}%
\fi
% ---------------------Transformaciones, mapeos, ... ---------------------------------------------
\iflibroproyecto
\glossary(Funciones){$\Phi$, $\Gamma$, $\Lambda$, $\Theta$,
                     $\Upsilon$, $\Omega$, $\Psi$}{Funciones o mapeos}%
\fi
% Composición entre transformaciones, mapeos, ...
\newcommand{\Comp}{\hspace{0.4pt}\circ\hspace{0.4pt}}%
% La flecha usada en los mapeos a-->b
\newcommand{\FlechaMap}{\hspace{-1pt}\mapsto\hspace{-1pt}}%--Esta macro no se considera que deba ir en el glosario
% ---------------------Caracter para indicar la no presencia de variable---------------------------
\newcommand{\NoVar}{\ifmmode\text{---}\else ---\fi}%
% -----Caracter para la separación de valores en el arreglo tabular propuesto----------------------
\newcommand{\CSep}{\thinspace\shortmid\thinspace}%
% -----Caracter para marcar los implicantes en el método de cubrimiento----------------------
\newcommand{\CMar}{\checkmark}%
% -----Caracter para cualquiera de las operaciones de disyunción o conjunción--------------------
\newcommand{\CDycCjc}{\star}%
% -----Operaciones de grupo --------------------
\newcommand{\OpBinGr}{\diamond}%
\newcommand{\OpUnGr}[1]{#1^{-1}}%
\newcommand{\IdGr}{e}%
% ----Macro para formatear los números de fila o columnas de tablas----------------------
\newcommand{\FNT}[1]{\textcircled{#1}}%{{\fboxsep1pt\framebox{#1}}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                             AMBIENTES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{demostracion}[1][Prueba]%
{\par\noindent\textbf{#1.}\nobreakspace}%
{\par}% Un ambiente para demostraciones
\iflibroproyecto
\newcounter{contejemplo}[chapter]%
\else
\newcounter{contejemplo}%
\fi
%\renewcommand{\thecontejemplo}{\arabic{chapter}.\arabic{contejemplo}}%
\newenvironment{ejemplo}{\vskip\baselineskip\par\noindent
\refstepcounter{contejemplo}%
\textbf{Ejemplo\nobreakspace\thecontejemplo}\nobreakspace}{\par}% Un ambiente para ejemplos
%\newenvironment{proof}%
%{\par\textbf{Prueba.}\nobreakspace}%
%{\par}% Un ambiente para Pruebas
\newtheorem{teorema}{Teorema}%                         Ambiente para teoremas 
%%\newtheorem{algoritmo}{Algoritmo}%                     Ambiente para algoritmos
\newtheorem{axioma}{Axioma}%                           Ambiente para axiomas
\newtheorem{corolario}{Corolario}%                     Ambiente para corolarios
\newtheorem{definicion}{Definici\'on}%                 Ambiente para definiciones
\newtheorem{lema}{Lema}%                               Ambiente para lemas
%%\newtheorem{proposicion}{Proposici\'on}%               Ambiente para propisiciones
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                             OTRAS DEFINICIONES MISCELANEAS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macro mara indicar el final de alguna cosa.
\newcommand{\Fin}{\nobreakspace\rule{0.5em}{0.5em}}%
% macro mara indicar el final de alguna cosa con espacio vertical agregado.
\newcommand{\FinEsp}[1][\baselineskip]{\Fin\vskip #1}%
